Triplets of local minima in a high-dimensional random landscape: Correlations, clustering, and memoryless activated jumps

We compute the distribution of triplets of stationary points in the energy landscape of the spherical p-spin model, by evaluating the quenched three-point complexity by means of the Kac-Rice formalism. We show the occurrence of transitions in the organization of stationary points in the landscape, identifying regions where local minima and saddles accumulate and cluster around other stationary points, thus displaying the presence of correlations in the landscape. We discuss the implications of these findings for the dynamical exploration of the energy landscape in the activated regime, specifying conditions under which transitions between local minima are expected to exhibit correlated rates and when, conversely, activated jumps are likely to be memoryless.

==> settings_custom.tex <==
% Shorthands
\def\new{\text{new}}
\def\iid{\text{i.i.d.}}
\newcommand{\extr}{\textrm{\textbf{extr}}}
\newcommand{\argmin}{\textrm{argmin}}
\newcommand{\prox}{\textrm{prox}}
\newcommand{\tot}{\textrm{tot}}

% Integral measures
\def\dd{\text{d}}

% Special functions
\def\sign{\text{sign}}
\def\erf{\text{erf}}
\def\relu{\text{relu}}


% Fixme and todo commands
\newcommand{\fixme}[1]{{\sffamily\normalsize\bfseries \underline{FIXME:} } { \color{red} #1} \\}

\newcommand{\todo}[1]{{\sffamily\normalsize\bfseries {\underline{\color{blue}TODO:}} } { \color{blue} #1}}

% Define theorem environment
\newtheorem{theorem}{Theorem}

%%Operators
\DeclareMathOperator{\Prox}{Prox}
\DeclareMathOperator*{\Extr}{Extr}
\DeclareMathOperator*{\Argmin}{argmin}

%%%%% Bold font
\newcommand{\bsA}{{\boldsymbol{\mathsf A}}}
\newcommand{\bG}{{\boldsymbol{G}}}
\newcommand{\bT}{{\boldsymbol{T}}}
\newcommand{\bOne}{{\boldsymbol{1}}}
\newcommand{\bR}{{\boldsymbol{R}}}
\newcommand{\bhR}{{\hat{\boldsymbol{R}}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bH}{{\boldsymbol{H}}}
\newcommand{\bA}{{\boldsymbol{A}}}
\newcommand{\bC}{{\boldsymbol{C}}}
\newcommand{\bS}{{\boldsymbol{S}}}
\newcommand{\bhS}{{\hat{\boldsymbol{S}}}}
\newcommand{\bU}{{\boldsymbol{U}}}
\newcommand{\bhU}{{\hat{\boldsymbol{U}}}}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bW}{{{\boldsymbol{{W}}}}}
\newcommand{\bw}{{\boldsymbol{w}}}
\newcommand{\bQ}{{\boldsymbol{Q}}}
\newcommand{\bV}{{\boldsymbol{V}}}
\newcommand{\bsQ}{{\boldsymbol{\mathsf Q}}}
\newcommand{\bsS}{{\boldsymbol{\mathsf S}}}
\newcommand{\bM}{{\boldsymbol{m}}}
\newcommand{\bhQ}{{\hat{\boldsymbol{Q}}}}
\newcommand{\bhV}{{\hat{\boldsymbol{V}}}}
\newcommand{\bhM}{{\hat{\boldsymbol{m}}}}
\newcommand{\bMM}{{{\boldsymbol{M}}}}
\newcommand{\bhMM}{{\hat{\boldsymbol{M}}}}
\newcommand{\bbb}{{\boldsymbol{b}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bbB}{{\boldsymbol{B}}}
\newcommand{\bF}{{\boldsymbol{F}}}
\newcommand{\bZ}{{\boldsymbol{Z}}}
\newcommand{\bY}{{\boldsymbol{Y}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bPi}{{\boldsymbol{\Pi}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bsigma}{{\boldsymbol{\sigma}}}
\newcommand{\blambda}{{\boldsymbol{\lambda}}}
\newcommand{\bomega}{{\boldsymbol{\omega}}}
\newcommand{\bzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bXi}{{\boldsymbol{\Xi}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\bX}{{\boldsymbol{X}}}
\newcommand{\bI}{{\boldsymbol{I}}}
\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\bff}{{\boldsymbol{f}}}
\newcommand{\be}{{\boldsymbol{e}}}
\newcommand{\beeta}{{\boldsymbol{\eta}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\bu}{{\boldsymbol{u}}}


% Matrix and vectors
\def\mat#1{\text{#1}}
\renewcommand{\vec}[1]{\bm{#1}}
